Pandemics Depress the Economy, Public Health Interventions Do Not: Evidence from the 1918 Flu

We study the impact of non-pharmaceutical interventions (NPIs) on mortality and economic activity across U.S. cities during the 1918 Flu Pandemic. The combination of fast and stringent NPIs reduced peak mortality by 50% and cumulative excess mortality by 24% to 34%. However, while the pandemic itself was associated with short-run economic disruptions, we find that these disruptions were similar across cities with strict and lenient NPIs. NPIs also did not worsen medium-run economic outcomes. Our findings indicate that NPIs can reduce disease transmission without further depressing economic activity, a finding also reflected in discussions in contemporary newspapers.

==> 91_mortality_on_manufacturing.tex <==
\appendix\section{The Effects of Mortality On Manufacturing Outcomes} \label{appendix:mortality}

In this appendix, we provide suggestive evidence that the severity of the 1918 Flu is correlated with lower economic activity using variation across U.S. states and cities. In particular, we use two approaches to estimate the impact of the 1918 Flu Pandemic on the real economy. The first approach is a standard difference-in-differences specification:
\begin{align}
    Y_{st} = \alpha_s + \tau_t + \sum_{j\neq 1914}\beta_j \, \mortality \, \mathbf{1}_{j=t} + \sum_{j\neq 1914} X_{s} \gamma_j \mathbf{1}_{j=t} + \varepsilon_{st} \label{spec1}
\end{align}
where $Y_{st}$ is an outcome such as log manufacturing employment in a local area $s$ in year $t$. The sequence of coefficients $\beta_j$ captures the dynamics of severely affected areas such as Pennsylvania relative to mildly affected areas such as Minnesota. Our baseline measure of local exposure to the 1918 pandemic is the local mortality rate from influenza and pneumonia per 100,000 inhabitants in 1918, $\mortality$. 

The identifying assumption behind estimation of \eqref{spec1} is parallel trends, i.e., $\mortality$ is not correlated with other time-varying, regional economic shocks. While there is significant geographic variation in the severity of the pandemic, studies using state-level variation in $\mortality$ argue that the spread of the virus was somewhat arbitrary and that regional variation in mortality was largely orthogonal to \textit{ex ante} economic conditions \citep{Brainerd2003}. Eastern states and cities were more severely affected, as the influenza arrived from Europe and travelled from east to west, but there is variation within U.S. regions. 

It is not obvious that $\mortality$ would be correlated with other economic shocks that differentially affected U.S. regions. Nevertheless, the period 1918-1921 witnessed a variety of macroeconomic shocks, most notably the end of WWI, a large agricultural boom and bust cycle, and a severe recession in 1920-21, \citep[see, e.g.,][]{Velde2020}. To account for potential differential exposure to these shocks, at the state level we control for the agriculture employment share, manufacturing employment share, urban population share, population, income per capita, and a war production dummy from \citet{Garrett2008}, represented by $X_s$ in \eqref{spec1}. At the city level, we control for 1910 population, manufacturing employment in 1914 to 1910 population, health expenditures in 1917 to 1910 population, city density in 1910, state agriculture employment share in 1910, and the state-level war production dummy. As in the main body of the text, all controls are measured before the 1918 pandemic and are always interacted with time fixed effects to control for time-varying shocks that are correlated with baseline differences across regions. We also present tests using a variety of additional controls.

A concern with exploiting variation in $\mortality$ is that mortality may be endogenous to economic outcomes. For example, higher mortality may have been a result of dire economic trajectories, so the parallel trends assumption may not be satisfied using variation in $\mortality$. To address this challenge, in our second approach, we instrument $\mortality$ with \textit{ex ante} exposure to military camps, similar to the empirical strategy suggested by \citet{Hilt2020} and also used by \citet{Meissner2020}.\footnote{\citet{Clay1918} also find that proximity to WWI base is associated with higher influenza mortality.} WWI military camps were important clusters and vectors of infection. For instance,  Fort Devens in Boston was the first cluster after the virus arrived from Europe, and it was transmitted to other camps via troop movements \citep{Crosby2003}.  Troops lived in close quarters, leading to rapid spread within camps, and troop movements disseminated virus across camps and to nearby cities. Camp location choice often also driven by historical military sites. For instance, Camp Funston in Kansas was built close to the historical military base in Fort Riley. Camp Colt in Pennsylvania was installed the historical Civil War site of Gettysburg. 

We collect information on the location and size of 40 military camps used on the continental U.S. in use during WWI (see Appendix \ref{appendix:data-military} for details). For each city, we construct a city-level instrument based on the weighted inverse distance to military camps:
\begin{align*}
Z_c =\sum_{j} \left[ \ln(camp \, size_{j} ) - \ln(dist_{c,j}) \right].
\end{align*}
$camp \, size_j$ is the average number of troops stationed in camp $j$ from July to September 1918, the onset of the second wave of the 1918 Flu Pandemic. $dist_{c,j}$ is the shortest path distance between city $c$ and camp $j$. In this formulation, larger camps receive a higher weight, and each camp's relative importance to city $c$ is weighted by the distance to city $c$. We also construct this instrument at the state-level using the distance between camp $j$ and the state centroid. 

Our military camps instrument $Z_c$ is a reasonably strong predictor of 1918 city-level influenza and pneumonia mortality at the city-level. The first-stage F-statistic of a regression of 1918 city level mortality on $Z_c$ is 19.9 without controls and 13.6 with baseline controls. At the state level, the first-stage F-statistics for the instrument are 3.25 without controls and 11.31 with controls. 

One potential concern with military camps exposure as an instrument for $\mortality$ is that military camps may have been close to locations with war production. During the war, these locations may have benefited from stronger growth in output. This concern is mitigated by examining the evolution of manufacturing outcomes from 1914, before the ramp-up in production, to 1919. Moreover, we find that controlling for an indicator variable for whether a state was heavily involved in war production \citep{Garrett2008} does not alter the results. Based on the measure from \citet{Garrett2008}, the location of military camps does not appear to be strongly related to major centers of war production.


\subsection{Results}

Panels (a) and (b) of \Cref{fig:state_city_mort_iv} present the results from estimation of \eqref{spec1} for state-level manufacturing employment and employment-to-population. The results show that high $\mortality$ exposure is associated with a significant decline in manufacturing employment and output from 1914 to 1919 census years. Both log employment and the employment-to-population ratio decline, indicating that the fall in employment is not only a direct consequence of deaths caused by the pandemic. Instead, the pandemic appears to be correlated with a broader disruption in manufacturing activity. 
 
Panel (c) of \Cref{fig:state_city_mort_iv} presents the city-level estimates of the impact of 1918 Flu Pandemic exposure on manufacturing outcomes. Because the OLS difference-in-differences estimates display a more severe negative pre-trend at the city-level, at the city level the estimates of $Mortality_{c,1918}$ instrumented by exposure to military camps can arguably be interpreted as a more reliable estimate of the economic impact of the pandemic. The instrumental variables difference-in-differences estimates at the city level indicate that the pandemic was associated with a decline in log manufacturing employment and output in high relative to low exposure cities. Further, the city-level instrumented estimates suggest there was a partial recovery in activity from 1919 to 1921 in more relative to less affected areas, but the relative decline seems nonetheless somewhat persistent.

Our findings on the negative effect of mortality during the 1918 Flu on manufacturing outcomes are in line with existing evidence on the adverse effect of the Flu  \citet{Barro2020}, \citet{Guimbeau2019}, \citet{Karlsson2014}, and \citet{Almond2006} However, it is important to note that our findings presented in this section are not necessarily robust to using other outcome variables. For instance, our evidence presented in \Cref{sec_npi} suggests that the disruptions from the Flu had largely passed by mid 1919. Further, \citet{Velde2020} carefully documents  that the impact of the Flu was rather short term than long term across a variety of different data sources. Thus, our evidence on manufacturing outcomes need to be evaluated with this caveat in mind.

Finally, the findings on mortality discussed in this section can also be considered jointly with the effect of NPIs. \Cref{fig:main_message} shows the city-level correlation between 1918 Flu mortality and the growth in manufacturing employment from 1914 to 1919 census years. As the figure reveals, higher mortality during the 1918 Flu is associated with a relative decline in economic activity. The figure further splits cities into those that were more and less aggressive in their use of NPIs. Cities that implemented stricter NPIs (green dots) tend to be clustered in the upper-left region (low mortality, high growth), while cities with more lenient NPIs (red dots) are clustered in the lower-right region (high mortality, low growth). This suggests that NPIs can play a role in attenuating mortality, but without reducing economic activity. If anything, cities with stricter NPIs during the pandemic perform better in the year after the pandemic.


==> tables/mortality_allcause_edr.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10}Intensity&       -0.90** &       -0.42   &       -1.17*  &               &               &               &               &               &               \\
                    &      (0.43)   &      (0.56)   &      (0.60)   &               &               &               &               &               &               \\
Speed               &               &               &               &       -4.35   &       -5.21*  &       -5.77*  &               &               &               \\
                    &               &               &               &      (3.26)   &      (2.95)   &      (2.98)   &               &               &               \\
High NPI            &               &               &               &               &               &               &     -120.65***&     -106.47** &     -167.38***\\
                    &               &               &               &               &               &               &     (38.94)   &     (45.15)   &     (41.75)   \\
\cmidrule{1-10} \RSq&        0.07   &        0.23   &        0.37   &        0.05   &        0.28   &        0.38   &        0.15   &        0.31   &        0.48   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
Add. controls       &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
\Oster              &           .   &        -.21   &        -1.3   &           .   &        -5.5   &        -6.3   &           .   &         -98   &        -188   \\


==> tables/mortality_allcause_peak_value.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10}Intensity&       -0.55***&       -0.38** &       -0.43*  &               &               &               &               &               &               \\
                    &      (0.11)   &      (0.17)   &      (0.23)   &               &               &               &               &               &               \\
Speed               &               &               &               &       -1.20   &       -1.08   &       -0.96   &               &               &               \\
                    &               &               &               &      (1.03)   &      (1.14)   &      (1.17)   &               &               &               \\
High NPI            &               &               &               &               &               &               &      -54.81***&      -47.82***&      -50.89***\\
                    &               &               &               &               &               &               &     (11.24)   &     (15.87)   &     (17.81)   \\
\cmidrule{1-10} \RSq&        0.25   &        0.35   &        0.37   &        0.03   &        0.29   &        0.32   &        0.28   &        0.43   &        0.44   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
Add. controls       &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
\Oster              &           .   &        -.19   &        -.32   &           .   &          -1   &        -.87   &           .   &         -42   &         -48   \\


==> tables/mortality_ip_edr.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10}Intensity&       -0.88** &       -0.59   &       -1.15** &               &               &               &               &               &               \\
                    &      (0.36)   &      (0.48)   &      (0.55)   &               &               &               &               &               &               \\
Speed               &               &               &               &       -3.41   &       -4.18   &       -4.54*  &               &               &               \\
                    &               &               &               &      (2.68)   &      (2.55)   &      (2.65)   &               &               &               \\
High NPI            &               &               &               &               &               &               &     -121.96***&     -111.03** &     -155.93***\\
                    &               &               &               &               &               &               &     (33.75)   &     (41.86)   &     (37.09)   \\
\cmidrule{1-10} \RSq&        0.09   &        0.31   &        0.40   &        0.04   &        0.33   &        0.39   &        0.20   &        0.40   &        0.52   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
Add. controls       &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
\Oster              &           .   &        -.46   &        -1.3   &           .   &        -4.4   &        -4.9   &           .   &        -104   &        -173   \\


==> tables/mortality_ip_edr_details.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10} \NPIIntensity&        -0.9** &        -0.6   &        -1.2** &               &               &               &               &               &               \\
                    &       (0.4)   &       (0.5)   &       (0.5)   &               &               &               &               &               &               \\
\NPISpeed           &               &               &               &        -3.4   &        -4.2   &        -4.5*  &               &               &               \\
                    &               &               &               &       (2.7)   &       (2.6)   &       (2.7)   &               &               &               \\
\HighNPI            &               &               &               &               &               &               &      -122.0***&      -111.0** &      -155.9***\\
                    &               &               &               &               &               &               &      (33.7)   &      (41.9)   &      (37.1)   \\
1917 I\&P mortality (per 100k)&               &         1.1***&         1.4***&               &         1.2***&         1.2***&               &         1.0** &         1.3***\\
                    &               &       (0.3)   &       (0.3)   &               &       (0.3)   &       (0.3)   &               &       (0.4)   &       (0.4)   \\
Longitude           &               &               &        -2.9   &               &               &        -2.1   &               &               &        -3.3*  \\
                    &               &               &       (2.2)   &               &               &       (2.5)   &               &               &       (1.9)   \\
Illiteracy          &               &               &        -6.9   &               &               &         3.9   &               &               &        -6.2   \\
                    &               &               &      (10.4)   &               &               &       (8.9)   &               &               &       (8.9)   \\
Medium coal-fired capacity&               &               &        73.8   &               &               &        75.6   &               &               &       115.1   \\
                    &               &               &      (87.0)   &               &               &      (83.1)   &               &               &      (86.7)   \\
High coal-fired capacity&               &               &       112.9   &               &               &       108.2   &               &               &       135.2*  \\
                    &               &               &      (74.5)   &               &               &      (71.2)   &               &               &      (75.3)   \\
\cmidrule{1-10}
\RSq                &        0.09   &        0.31   &        0.40   &        0.04   &        0.33   &        0.39   &        0.20   &        0.40   &        0.52   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
\Oster              &           .   &        -.46   &        -1.3   &           .   &        -4.4   &        -4.9   &           .   &        -104   &        -173   \\
Baseline controls   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
   \bottomrule


==> tables/mortality_ip_peak_value.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10}Intensity&       -0.52***&       -0.41** &       -0.44*  &               &               &               &               &               &               \\
                    &      (0.10)   &      (0.16)   &      (0.22)   &               &               &               &               &               &               \\
Speed               &               &               &               &       -1.11   &       -0.98   &       -0.90   &               &               &               \\
                    &               &               &               &      (0.95)   &      (1.09)   &      (1.13)   &               &               &               \\
High NPI            &               &               &               &               &               &               &      -52.05***&      -47.27***&      -49.23***\\
                    &               &               &               &               &               &               &     (10.33)   &     (15.06)   &     (16.95)   \\
\cmidrule{1-10} \RSq&        0.27   &        0.35   &        0.37   &        0.03   &        0.26   &        0.31   &        0.30   &        0.42   &        0.44   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
Add. controls       &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
\Oster              &           .   &        -.25   &        -.36   &           .   &        -.94   &        -.82   &           .   &         -42   &         -47   \\


==> tables/mortality_ip_peak_value_details.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10} \NPIIntensity&        -0.5***&        -0.4** &        -0.4*  &               &               &               &               &               &               \\
                    &       (0.1)   &       (0.2)   &       (0.2)   &               &               &               &               &               &               \\
\NPISpeed           &               &               &               &        -1.1   &        -1.0   &        -0.9   &               &               &               \\
                    &               &               &               &       (0.9)   &       (1.1)   &       (1.1)   &               &               &               \\
\HighNPI            &               &               &               &               &               &               &       -52.1***&       -47.3***&       -49.2***\\
                    &               &               &               &               &               &               &      (10.3)   &      (15.1)   &      (17.0)   \\
1917 I\&P mortality (per 100k)&               &         0.1   &         0.1   &               &         0.2** &         0.1   &               &         0.1   &         0.1   \\
                    &               &       (0.1)   &       (0.1)   &               &       (0.1)   &       (0.1)   &               &       (0.1)   &       (0.1)   \\
Longitude           &               &               &        -0.4   &               &               &         0.1   &               &               &        -0.4   \\
                    &               &               &       (0.7)   &               &               &       (0.8)   &               &               &       (0.6)   \\
Illiteracy          &               &               &         0.6   &               &               &         4.5   &               &               &         1.5   \\
                    &               &               &       (4.0)   &               &               &       (3.0)   &               &               &       (3.3)   \\
Medium coal-fired capacity&               &               &         3.8   &               &               &         0.4   &               &               &        15.5   \\
                    &               &               &      (31.9)   &               &               &      (30.4)   &               &               &      (30.9)   \\
High coal-fired capacity&               &               &        18.2   &               &               &        16.2   &               &               &        24.9   \\
                    &               &               &      (27.4)   &               &               &      (26.8)   &               &               &      (26.6)   \\
\cmidrule{1-10}
\RSq                &        0.27   &        0.35   &        0.37   &        0.03   &        0.26   &        0.31   &        0.30   &        0.42   &        0.44   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
\Oster              &           .   &        -.25   &        -.36   &           .   &        -.94   &        -.82   &           .   &         -42   &         -47   \\
Baseline controls   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
   \bottomrule


==> tables/mortality_markel_edr.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10}Intensity&       -0.98** &       -0.63   &       -1.27** &               &               &               &               &               &               \\
                    &      (0.37)   &      (0.49)   &      (0.56)   &               &               &               &               &               &               \\
Speed               &               &               &               &       -4.12   &       -4.78*  &       -5.12*  &               &               &               \\
                    &               &               &               &      (2.83)   &      (2.68)   &      (2.77)   &               &               &               \\
High NPI            &               &               &               &               &               &               &     -135.62***&     -122.45***&     -172.63***\\
                    &               &               &               &               &               &               &     (34.83)   &     (43.09)   &     (38.34)   \\
\cmidrule{1-10} \RSq&        0.11   &        0.30   &        0.40   &        0.05   &        0.32   &        0.39   &        0.22   &        0.40   &        0.53   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
Add. controls       &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
\Oster              &           .   &        -.46   &        -1.4   &           .   &          -5   &        -5.5   &           .   &        -114   &        -192   \\


==> tables/mortality_markel_peak_value.tex <==
                    &         (1)   &         (2)   &         (3)   &         (4)   &         (5)   &         (6)   &         (7)   &         (8)   &         (9)   \\
\cmidrule{1-10}Intensity&       -0.57***&       -0.45** &       -0.48** &               &               &               &               &               &               \\
                    &      (0.10)   &      (0.17)   &      (0.22)   &               &               &               &               &               &               \\
Speed               &               &               &               &       -1.18   &       -1.02   &       -0.98   &               &               &               \\
                    &               &               &               &      (0.98)   &      (1.07)   &      (1.11)   &               &               &               \\
High NPI            &               &               &               &               &               &               &      -54.48***&      -48.73***&      -50.08***\\
                    &               &               &               &               &               &               &     (10.84)   &     (15.89)   &     (17.74)   \\
\cmidrule{1-10} \RSq&        0.30   &        0.36   &        0.39   &        0.03   &        0.26   &        0.32   &        0.30   &        0.41   &        0.45   \\
Number of cities    &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   &          46   \\
Add. controls       &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   &           -   &         Yes   &         Yes   \\
\Oster              &           .   &        -.25   &        -.37   &           .   &        -.97   &        -.91   &           .   &         -43   &         -46   \\

